Mixture-Net: Low-Rank Deep Image Prior Inspired by Mixture Models for Spectral Image Recovery

This paper proposes a non-data-driven deep neural network for spectral image recovery problems such as denoising, single hyperspectral image super-resolution, and compressive spectral imaging reconstruction. Unlike previous methods, the proposed approach, dubbed Mixture-Net, implicitly learns the prior information through the network. Mixture-Net consists of a deep generative model whose layers are inspired by the linear and non-linear low-rank mixture models, where the recovered image is composed of a weighted sum between the linear and non-linear decomposition. Mixture-Net also provides a low-rank decomposition interpreted as the spectral image abundances and endmembers, helpful in achieving remote sensing tasks without running additional routines. The experiments show the MixtureNet effectiveness outperforming state-of-the-art methods in recovery quality with the advantage of architecture interpretability.

==> Deep Unmixing based neural network/Tables/table1.tex <==
\begin{table}[b!]
\scriptsize
\renewcommand{\arraystretch}{1.0}
\caption{Denoising Quantitative Results for Pavia University}
\label{tab:denoising}
\centering
\resizebox{1\columnwidth}{!}{%
\setlength\tabcolsep{0.05cm}
\begin{tabular}{llllllllll} 
\toprule 
\begin{tabular}[c]{@{}c@{}}Noise\\ $\sigma$\end{tabular} & Metric &\dcheck{Input} & BM3D & FORPDN & HyRes & DIP &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}SURE\\ CNN\end{tabular}} & DS2DP &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Mixture\\-Net\end{tabular}}\\
\bottomrule
\midrule
\multirow{2}{*}{{$\frac{100}{255}$}} & $\uparrow$PSNR &\dcheck{$8.130$} & {$29.14$} & $26.03$ & $28.41$ & $26.47$ &\underline{$29.62$} & $27.54$ & $\mathbf{30.95}$\\ 
&$\downarrow$SSIM &\dcheck{$0.025$} & {$0.754$} & $0.597$ & $0.738$ & $0.683$ &\underline{$0.802$} &$0.718$ & $\mathbf{0.869}$\\ 
\midrule 
\multirow{2}{*}{$\frac{50}{255}$} & $\uparrow$PSNR &\dcheck{$14.15$} & {$32.97$} & $30.44$ & $31.78$ & $30.69$ &\underline{$33.29$} & $32.12$ & $\mathbf{34.47}$\\ 
&$\downarrow$SSIM &\dcheck{$0.102$} & $0.881$ & $0.799$ & $0.855$ & $0.846$ &\underline{$0.905$} & $0.896$ & $\mathbf{0.942}$\\ 
\midrule 
\multirow{2}{*}{$\frac{25}{255}$} & $\uparrow$PSNR &\dcheck{$20.17$} &\underline{$36.48$} & $34.34$ & $35.35$ & $34.48$ & {$36.09$} & $35.55$ & $\mathbf{36.99}$\\ 
&$\downarrow$SSIM &\dcheck{$0.286$} & $0.942$ & $0.906$ & $0.927$ & $0.917$ & $0.945$ &\underline{$0.951$}& $\mathbf{0.965}$\\ 
\bottomrule
\end{tabular} }
\end{table}

==> Deep Unmixing based neural network/Tables/table2_3.tex <==
\begin{table}[ht!]
\scriptsize
\renewcommand{\arraystretch}{1.00}
\caption{Single Hyperspectral Super-Resolution Quantitative Results for Pavia Center}
\label{tab:sematic_depth}
\centering
\resizebox{1\columnwidth}{!}{%
\setlength\tabcolsep{0.1cm}
\begin{tabular}{lcccccc} 
\toprule 
Method & $d$ & SAM$\downarrow$ & RMSE$\downarrow$ & ERGAS$\downarrow$ & PSNR$\uparrow$ & SSIM $\uparrow$\\
\midrule 
Bicubic & 4 & 6.1399 & 0.0437 & 6.8814 & 27.5874 & 0.6961\\\midrule 
EDSR & 4 & 5.8657 &0.0379 & 6.0199 & 28.7981& 0.7722\\ 
RCAN & 4 & 5.9785 &0.0376 & 6.0485 & 28.8165& 0.7719\\ 
SAN & 4 & 5.9590 &0.0374 & 5.9903 & 28.8554& 0.7740\\ 
\midrule 
3DCNN & 4 & 5.8669 &0.0396 & 6.2665 & 28.4114& 0.7501\\ 
GDRRN & 4 & 5.4750 &0.0393 & 6.2264 & 28.4726& 0.7530\\ 
SSPSR & 4 &\underline{5.4612} &\underline{0.0362} &\textbf{5.8014} &\underline{29.1581} &\underline{0.7903}\\
\midrule 
DIP& 4 & 6.2665 &0.0410 & 6.4845 & 28.1061& 0.7365\\ 
Mixture-Net & 4 &\textbf{4.2120} &\textbf{0.0352} &\underline{5.8084} &\textbf{29.914}&\textbf{0.8396}\\
\bottomrule 
\midrule 
Bicubic & 8 & 7.8478 & 0.0630 & 4.8280 & 24.5972 & 0.4725\\\midrule 
EDSR & 8 & 7.8594 & 0.05983 & 4.6359 & 25.0041 & 0.5130\\
RCAN & 8 & 7.9992 & 0.0604 & 4.6930 & 24.9183 & 0.5086\\
SAN & 8 & 8.0371 & 0.0609 & 4.7646 & 24.8485 & 0.5054\\
\midrule 
3DCNN & 8 & 7.6878 & 0.0605 & 4.6469 & 24.9336 & 0.5038\\
GDRRN & 8 & 7.3531 & 0.0607 & 4.6220 & 24.8648 & 0.5014\\
SSPSR &8 &\underline{7.3312} &\underline{0.0586} &\underline{4.5266} &\underline{25.1985} &\underline{0.5365}\\
\midrule 
DIP & 8 &7.9281 &0.0618 &4.7366 &24.7252 &0.4963\\
Mixture-Net & 8 &\textbf{6.7855} &\textbf{0.0485} &\textbf{4.0015} &\textbf{26.9041} &\textbf{0.7148}\\
\bottomrule 
\end{tabular} }
\end{table}
\begin{table}[ht!]
\scriptsize
\renewcommand{\arraystretch}{1.00}
\caption{ Single Hyperspectral Super-Resolution Quantitative Results for Stuff-Toys }
\label{tab:sematic_depth_CAVE}
\centering
\resizebox{1\columnwidth}{!}{%
\setlength\tabcolsep{0.1cm}
\begin{tabular}{lcccccc} 
\toprule 
Method & $d$ & SAM$\downarrow$ & RMSE$\downarrow$ & ERGAS$\downarrow$ & PSNR$\uparrow$ & SSIM $\uparrow$\\
\midrule 
Bicubic & 4 & 4.1759 & 0.0212 & 5.2719 & 34.7214 & 0.9277\\\midrule 
EDSR & 4 & 3.5499 & 0.0149 & 3.5921 & 38.1575 & 0.9522\\
RCAN & 4 & 3.6050 & 0.0142 & 3.4178 & 38.7585 & 0.9530\\
SAN & 4 & 3.5951 & 0.0143 & 3.4200 & 38.7188 & 0.9531\\
\midrule 
3DCNN & 4 & 3.3463 & 0.0154 & 3.7042 & 37.9759 & 0.9522\\
GDRRN & 4 &\underline{3.4143} & 0.0145 & 3.5086 & 38.4507 & 0.9538\\
SSPSR & 4 &\textbf{3.1846} & 0.0138 & 3.3384 &\underline{39.0892} & 0.9553\\
\midrule
DIP & 4 & 8.4935 &\underline{0.0124} &\underline{ 2.5358} & 38.1329 &\underline{0.9631}\\
Mixture-Net &4& 5.3285&\textbf{0.0110} &\textbf{2.1997} &\textbf{39.1640} &\textbf{0.9821}\\
\bottomrule 
\midrule 
Bicubic & 8 & 5.8962 & 0.0346 & 4.2175 & 30.2056 & 0.8526\\\midrule 
EDSR & 8 & 5.6865 & 0.0279 & 3.3903 & 32.4072 & 0.8842\\
RCAN & 8 & 5.9771 & 0.0268 & 3.1781 & 32.9544 & 0.8884\\
SAN & 8 & 5.8683 & 0.0267 & 3.1437 & 33.0012 & 0.8888\\
\midrule 
3DCNN & 8 &\underline{5.0948} & 0.0292 & 3.5536 & 31.9691 & 0.8863\\ 
GDRRN & 8 & 5.3597 & 0.0280 & 3.3460 & 32.5763 & 0.8890\\
SSPSR & 8 &\textbf{4.4874} & 0.0257 & 3.0419 &
\underline{33.4340} & 0.9010\\
\midrule
DIP & 8 & 8.3342 &\underline{0.0231} &\underline{2.3697}& 32.7324&\underline{0.9291}\\
Mixture-Net &8& 5.5027&\textbf{0.0208} &\textbf{2.1061} &\textbf{33.6270} &\textbf{0.9432}\\
\bottomrule 
\end{tabular} }
\end{table}


==> Deep Unmixing based neural network/Tables/table4.tex <==
\begin{table}[h!]
\scriptsize
% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1.25}
\caption{Compressive Spectral Imaging Reconstruction Quantitative Results}
\label{tab:compressive_spectral_reconstruction}
\centering
\resizebox{1\columnwidth}{!}{%
\setlength\tabcolsep{0.05cm}
\begin{tabular}{lllllll} 
\multicolumn{7}{c}{\textbf{KAIST}}\\
\toprule\multicolumn{1}{c}{\textbf{Metric}} &\multicolumn{1}{c}{\textbf{PnP}} &\multicolumn{1}{c}{\textbf{DNU}} &\multicolumn{1}{c}{\textbf{AE}} &\multicolumn{1}{c}{\textbf{TL-DIP}} &\multicolumn{1}{c}{\textbf{\dcheck{JR2net}}} &\multicolumn{1}{c}{\textbf{Mixture-Net}}\\
\bottomrule
\midrule
$\uparrow$PSNR & 
$29.8\pm2.6$ &	
$32.6\pm1.8$ & 
$37.9\pm1.1$ & 
$32.8\pm0.9$ &
\dcheck{\underline{$39.1\pm2.5$}} & 	
$\mathbf{40.3\pm2.6}$ \\ 
$\uparrow$SSIM & 
$0.92\pm0.02$ & 
$0.91\pm0.01$ &	
$0.96\pm0.01$ &		
$0.92\pm0.01$ &
\dcheck{\underline{$0.97\pm0.02$}}& 
$\mathbf{0.99\pm0.01}$ \\ 
$\downarrow$SAM & 
$10.9\pm4.2$ & 
$12.9\pm1.8$ &	
$9.20\pm2.9$ &	
$12.4\pm2.7$ &	
\dcheck{\underline{$6.00\pm2.3$}} &	
$\mathbf{3.26\pm1.1}$\\ 
\midrule 
\multicolumn{7}{c}{\textbf{ARAD}}\\
\toprule
$\uparrow$PSNR & 
$31.5\pm4.5$ &	
$29.5\pm4.5$ &	 
$33.5\pm4.4$ &
$35.8\pm3.8$ &	
\dcheck{\underline{$36.5\pm4.6$}} &	
$\mathbf{39.1\pm4.1}$ \\ 
$\uparrow$SSIM & 
$0.83\pm0.08$ &	
$0.82\pm0.09$ &	
$0.90\pm0.05$ &	
$0.95\pm0.03$ &	
\dcheck{\underline{$0.97\pm0.01$}} &	
$\mathbf{0.98\pm0.01}$ \\ 
$\downarrow$SAM & 
$6.94\pm2.7$ &	
$8.26\pm3.1$ &	
$5.50\pm1.7$ &	
$4.45\pm2.5$ &	
\dcheck{\underline{$2.85\pm0.95$}} &	
$\mathbf{2.04\pm0.53}$\\
\bottomrule
\end{tabular}}
\end{table}


==> Deep Unmixing based neural network/tikz/figure11.tex <==
\begin{figure}[tb!]
\centering
\includegraphics[width=1\linewidth]{Figures/Figure11/mi_imagen.pdf}\caption{\textit{(left)} RGB Ground truth and estimated Fake image. \textit{(Top right)} Two obtained features interpreted as the abundances. \textit{(Bottom right)} Binary maps  after applying a threshold, identifying the differences in the materials. }\label{fig:kaistcomp}
\end{figure}

==> Deep Unmixing based neural network/tikz/figure4.tex <==
\begin{figure}[b!]
\centering
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\node[inner sep=0pt] (Abun) at (0\linewidth,0){\includegraphics[width=1\linewidth]{Figures/Figure4/EfectoNoLinearV2.pdf}};
\node at (-0.25\linewidth,2.3cm){$\uparrow$\textbf{PSNR [dBs] }};
\node at (0.25\linewidth,2.3cm){$\downarrow$\textbf{SAM [Degrees] }};
\node at (-0.25\linewidth,-1.4cm) {Rank };
\node at (0.25\linewidth,-1.4cm) {Rank};
\end{tikzpicture}
\caption{\dcheck{Quantitative performance in terms of PSNR {(\textit{left})} and SAM {(\textit{right})} when using the linear block-layer, i.e., $\lambda=0$ in~\eqref{eq:eq7}, and when including the non-linearity block-layer with {$\lambda=0.7$. The rank value varies in the range $[3,4,5,6,7,8,9,10, 15, 20]$. The non-linearity block-layer is composed of two consecutive spatial-spectral networks presented in~\cite{wang2019hyperspectral}, with the learning rate set to $lr = 1e^{-3}$.}} 
}
\label{fig:rank_behaviour}
\end{figure}
 

==> Deep Unmixing based neural network/tikz/figure5.tex <==
\begin{figure}[ht!]
\centering
\includegraphics[width=0.48\linewidth]{Figures/Figure5/NumberOfBlocks.pdf}
\includegraphics[width=0.48\linewidth]{Figures/Figure5/IntermediateBlocks.pdf}
\caption[justification=justified]{\dcheck{(\textit{left}) Mixture-Net performance, varying the number of interpretable deep-blocks in the range $[1-5]$ for single and multiple losses. (\textit{right}) Recovered image quality at each intermediate deep-block when fixing five deep-blocks.}}
\label{fig:my_deepblocks}
\end{figure}
